Timeline Design Space for Immersive Exploration of Time-Varying Spatial 3D Data

Timelines are common visualizations to represent and manipulate temporal data, from historical events storytelling to animation authoring. However, timeline visualizations rarely consider spatio-temporal 3D data (e.g. mesh or volumetric models) directly, which are typically explored using 3D visualizers only displaying one time-step at a time. In this paper, leveraging the increased workspace and 3D interaction capabilities of virtual reality, we propose to use timelines for the visualization of 3D temporal data to support exploration and analysis. First, we propose a timeline design space for 3D temporal data extending the timeline design space proposed by Brehmer et al. The proposed design space adapts the scale, layout and representation dimensions to account for the depth dimension and how 3D temporal data can be partitioned and structured. In our approach, an additional dimension is introduced, the support, which further characterizes the 3D dimension of the visualization. To complement the design space and the interaction capabilities of VR systems, we discuss the interaction methods required for the efficient visualization of 3D timelines. Then, to evaluate the benefits of 3D timelines, we conducted a formal evaluation with two main objectives: comparing the proposed visualization with a traditional visualization method; exploring how users interact with different 3D timeline designs. Our results showed that time-related tasks can be achieved more comfortably using timelines, and more efficiently for specific tasks requiring the analysis of the surrounding temporal context. Though the comparison between the different timeline designs were inconclusive, participants reported a clear preference towards the timeline design that did not occupy the vertical space. Finally, we illustrate the use of the 3D timelines to a real use-case on the analysis of biological 3D temporal datasets.

==> additional.tex <==
\begin{figure*}[h]
\centering
\subfloat[][Comfort]{\includegraphics[width=0.45\textwidth]{Pictures/Qcomfort_cropped.pdf}} \hspace{0.5cm}
\subfloat[][Efficiency]{\includegraphics[width=0.45\textwidth]{Pictures/Qefficiency_cropped.pdf}}\\

\includegraphics[width=0.3\textwidth]{Pictures/Subjective_Scale.pdf}
\caption{Subjective results for each timeline design and task. (a) Ranking results for the question ``What condition felt the most comfortable for this task?''. (b) Ranking results for the question ``What condition seemed the most efficient for this task?'' }\label{fig:Qcomfort}
\end{figure*} 


\begin{table}[h]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}\label{table:designEvaluation}

==> brainstorm.tex <==

\pagebreak 
\section{brainstorm}
See Fig.\ref{fig:fig}
\subsection{Why are we using timelines?}

\begin{figure}[h!]
\centering
\includegraphics[width=0.477\textwidth]{Pictures/fig.png}
\caption{Fig}\label{fig:fig}
\end{figure} 

We have sequences of chronological 3D models, some punctual events, some lasting events, values evolving over time. 
%
Timelines show the temporal context of 1 object.
%
Displaying the 3D object at each time point of the timeline could be relevant to visualize the evolution of the object in terms of shape or other attributes.


Main issues that could be solved with timelines:

\begin{itemize}
    \item Visualization of punctual events, such as fusion, division, transformation
    \item Visualization of the evolution of an object, of a group of objects
    \item Navigation in time
    \item Comparison tasks
\end{itemize}


\subsection{What can a 3D layout provide?}

\toDo{4.0: immersive environment}
Benefits of 3D environment :
\begin{itemize}
    \item Visualization of 3D items or 3D spaces via stereoscopic display. Adding depth cues in desktop visualization could be enough, however it could rely on size or color transformation, which we want to avoid in our use cases, hence the use of VR.
    \item Exploration the 3D items in immersive environment $\rightarrow$ navigation and interaction
    \item More space = more timelines $\rightarrow$ good for comparison task, between 2 time points or 2 objects
\end{itemize}


Benefits of a 3D layout: 
\begin{itemize}
    \item Curve to see everything without scrolling but just turning head (easier navigation)
    \item Spiral to align events or $\neq$ objects $\rightarrow$ \emph{comparison task}
    \item Spiral also compacts
    \item Supplementary dimension to encode data? $\rightarrow$ Should be on an intuitive display, such as a curve with appearing 0-line and we change stuff on Z-dimension for instance
\end{itemize}


\subsection{What kind of data are we displaying?}

\begin{itemize}
    \item Spatial data: cells, endosomes, more or less sparse. Unique objects nonetheless, that can be interesting as groups
    \item Quantitative values: evolving values over time, values changing with events
    \item Qualitative information : groups, cell ID, stuff
    \item Hierarchy through division and fusion
\end{itemize}

\section{Display and Interaction}

\subsection{How do we display the data, considering we have a timeline?}


Design details \cite{brehmer_timelines_2017}
\begin{description}
    \item[Representation : ]{
        \begin{itemize}
            \item linear (classic) : generic and straightforward, you can represent any timeline with it and pay the price after
            \item 3D curve : adaptation of linear rep helping in getting time points closer. The curve you can get will depend on the amount of time points though
            \item helicoid : can handle a lot of time points, all close together. Align with cyclical events? Explore quickly through time by jumping from row to row (kinda replaces the role of juxtaposed layout). Oppressing or immersive ? problem if it gets too high or underground. cyclic events, fun.
            \item spherical: spiralling around a sphere. Everything is as close as possible ++comparison. Limited in terms of time points. Same limitations than with a  2d spiral, cyclical but the inner circles get smaller and smaller, not optimal for visualizing cycles
        \end{itemize}
    }
    \item[Scale: ] {
        \begin{itemize}
            \item basically nothing changes
            \item chronological/sequential since our time points are equally separated
        \end{itemize}
    }
    \item[Layout: ] {
        \begin{itemize}
            \item multiple timelines juxtaposed, either 2 daughter cells coming from one, or just 2 cells compared:
                comparison object by object. takes a lot of space to separate them correctly
            \item grouping objects: spatial information on objects, neighbouring relations and such
            \item zone: less of an object approach, might not be able to follow the behaviour of objects. Though useful if waiting an event in a specific place. -> spatial information, not on the objects but on their context
        \end{itemize}
    }
\end{description}



Other display information:
\begin{itemize}
    \item 3D meshes as time points
    \item line with gradient colors
    \item specific encoding of a spatial dimension ?
    \item adding trajectory information, maybe juxtaposed ?
\end{itemize}




\subsection{How do we explore the timeline?}

Classic interactions
\begin{itemize}
    \item  detail-on-demand on each time point $\rightarrow$ pointer
    \item level-of-detail $\rightarrow$ bimanual interaction, bringing closer or farther 2 time points
    \item move the timeline to get the current node in front of you
    \item alignment tools (selecting 2 objects, aligning the timeline relatively)
    \item filtering interface, in time by value (make nodes smaller, or disappear, but then need time info somewhere)
\end{itemize}

3D layout oriented interactions
\begin{itemize}
    \item cut-away view and rotation done equally on each time point
\end{itemize}

\subsection{Juxtaposition and comparison}
Multiple selection
\begin{itemize}
    \item Brushing
    \item Select one by one with a pointer
    \item Extend a zone using widgets
    \item Select the neighbours directly on the timeline
\end{itemize}

Juxtaposition
\begin{itemize}
    \item one under the other
    \item one behind the other
    \item all object selected counted as 1 in a global timeline
\end{itemize}

    
\section{Drawbacks and difficulties}

Position/trajectory information is pretty much lost
\begin{itemize}
    \item Juxtapose with trajectory ?
\end{itemize}

Lack of spatial context
\begin{itemize}
    \item Widgets to expand zone ?
    \item Adding every cell selected?
    
\end{itemize}


\section{Biology Use cases}
Annotation

Hierarchy errors

\section{non expert user experiment}
arbitrary task, well justified, yet not needing previous knowledge on the data
transmissible to biology tasks



\vspace{10cm}

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

